SONNI: Secure Oblivious Neural Network Inference

In the standard privacy-preserving Machine learning as-a-service (MLaaS) model, the client encrypts data using homomorphic encryption and uploads it to a server for computation. The result is then sent back to the client for decryption. It has become more and more common for the computation to be outsourced to third-party servers. In this paper we identify a weakness in this protocol that enables a completely undetectable novel model-stealing attack that we call the Silver Platter attack. This attack works even under multikey encryption that prevents a simple collusion attack to steal model parameters. We also propose a mitigation that protects privacy even in the presence of a malicious server and malicious client or model provider (majority dishonest). When compared to a state-of-the-art but small encrypted model with 32k parameters, we preserve privacy with a failure chance of 1.51 x 10^-28 while batching capability is reduced by 0.2%. Our approach uses a novel results-checking protocol that ensures the computation was performed correctly without violating honest clients' data privacy. Even with collusion between the client and the server, they are unable to steal model parameters. Additionally, the model provider cannot learn any client data if maliciously working with the server.

==> 06-experiments.tex <==
\section{Experiments \label{sec:experiments}}

In this section,...

\subsection{Experimental Setup}

\subsection{Results}

==> old/old_02-introduction.tex <==
\lnote{ old outline below:


Intro 

ML as service is important 
Privacy important  
Privacy is often thought of from client perspective, they have an input x and they want to apply ML model to it to get f(x.t) 
There is an aspect of privacy for the ML model itself 
Typically handled by the server doing the computation locally 
Not feasible as ML models get bigger 
Putting static resources for provide ML as service becomes challenging 
We want to be able to use commercially available servers that you can request when needed (e.g., because your servers are heavily loaded) 
Problem is that these commercially available servers will learn the ML model without proper care.  
Server does not want this 
Problem is to provide ML as service while providing privacy to client for input x and privacy for server for model M 
Terminology: Mercenary  
Permitted operations: polynomial, convolution and multiplication  
 
Structure of the paper 

\begin{itemize}
    \item First algorithm: No Collusion of any kind 
\item Secret key only with client  
\item Algorithm for 
\item Polynomial computation 
\item Convolution computation  
\item Matrix multiplication  
\item Problems 
\item Collusion will reveal XX 
\item Algorithm 2.1: collusion between mercenaries and clients 
\item Threshold cryptography with client and sever holding a key and both required for decryption 
\item Client and server both maintain the privacy 
\item How can mercenaries try to break server privacy by cooperation with clients    
\item Mercenary sends Enc(parameter) to server which decrypts and sends to client there by violate server privacy 
\item Solution  
\item 3 key approach if ok to learn f(x) when f(x) is a classification problem.  
\item Random multiplication 
\item Keep a portion of the tree on server itself and not delegate 
\item Split into multiple polynomials so that parameters learnt in one invocation are different from another invocation 
\item How can mercenaries try to break client privacy by cooperation with server  

\end{itemize}
 
Limitations and future work 
Max operation not yet supported 
}


==> old/old_03-approach.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/overview.png}
    \caption{rough draft of overview figure}
    \label{fig:overview}
\end{figure}

\section{\ourmethod}
In this section, we introduce our secure and private function computation protocol, \ourmethod. 

\subsection{Problem Statement}
We tackle the novel problem of MLaaS in a distributed setting. We identify three types of processes. The client process holds some secret data $x$ and wants to obtain \fnoutput where $f$ is a parameterized function held by the server process. The server holds secret parameters to $f$ that we denote as $t$ \lnote{ make t a vector?}. The server aims to learn nothing from the protocol while maintaining the privacy of $t$. 

The third type of process is hired by the server to compute \fnoutput obliviously. We call these mercenary processes. Mercenary processes should not learn $x$, $t$, or \fnoutput. 

\subsection{Protocol Overview}
Fully homomorphic encryption (FHE) is popular for its ability to evaluate neural networks in a privacy-preserving manner. We distribute the workload over all the mercenary processes to increase parallelism while maintaining privacy. Figure \ref{fig:overview} shows our protocol overview. Threshold FHE \cite{chowdhury2022efficient} is used with two secret key shares. One is held by the client and one is held by the server. Both are needed to decrypt any ciphertexts. This setup ensures that collusion attacks fail to break either the client or the server's privacy. The mercenary processes hold no secret key shares and instead perform \lnote{the bulk of? all of?} the homomorphic arithmetic operations described in the following subsections.

After processing ciphertexts, the resultant ciphertexts are sent to the server which applies its share of the secret key before sending the results to the client. The client then decrypts the results and obtains $f(x)$

\subsection{Polynomial Evaluation}
Polynomial evaluation is vital in privacy-preserving machine learning for its application in replacing activation functions in the homomorphic space ~\cite{}. In a centralized setting, a single process may evaluate a polynomial through a series of homomorphic multiplications and additions. This can be done in a multiplicative depth of $log(d)$ for a degree $d$ polynomial. Our approach simultaneously distributes the work among all mercenary processes while providing collusion resistance to prevent any process from learning the secret parameter values of the function.

The server first factors the polynomial by dividing it by a random binomial. This is repeated until it is divided in $n$ components. These components are encrypted and sent to the mercenary processes, one component each, along with the ciphertext representing the input to the function. The mercenary processes can now evaluate the polynomial by computing their portion of the polynomial and sending the result to the next process in the chain. Collusion attacks fail here because the original polynomial cannot be reconstructed unless all components are pooled together. Therefore, all mercenary processes would need to collude with the client to break the privacy of the server.

The multiplicative depth of this protocol is $d$ due to the binomial evaluations.

\subsection{Matrix Multiplication}
To evaluate linear layers of neural networks (a fundamental portion of many architectures), matrix multiplication is needed. \lnote{can I cite myself here? It seems important for the discussion} Sperling \cite{sperling2022heft} showed that the homomorphic matrix-vector multiplication operation that is most efficient for a large number of vector samples is the so-called SIMD matrix multiplication method \cite{engelsma2022hers}.

The basic idea behind the SIMD matrix multiplication is to have each value in the left matrix encrypted as a ciphertext where every slot of the ciphertext has the same value. The right matrix is encrypted over the rows. Then, by multiplying the appropriate ciphertexts and summing together the result, the operation is complete with a multiplicative depth of $1$ and no rotation operations needed.

In \ourmethod, the left matrix represents the model's weights and the right represents the input (batched) to the linear layer. This work can also be distributed by each process computing a subset of the needed multiplications and then pooling together their values via message-passing.

\subsection{Convolution}
Juvekar et al. proposed a homomorphic convolution operation that operates on ciphertexts \cite{juvekar2018gazelle}. For a kernel of size $f_w \times f_h$, $f_w f_h - 1$ rotations and additions are needed, along with $f_w f_h$ multiplications. Their representation batches entire images into single ciphertexts. 
\lnote{our method is actually quite different and I believe novel. I should create a figure showing what it does.} Our representation batches along rows of matrices, however, the algorithm is otherwise unchanged. Data about the number of homomorphic operations is shown in Table \ref{tab:complexity}.

Each of the multiplications and rotations performed in the homomorphic convolution are independent of each other and can therefore be done in parallel.

\subsection{A Note on Pooling}
In traditional CNN architecture, max pooling layers are used. Dathathri et al. demonstrated the viability of average pooling as a replacement \cite{dathathri2019chet}. This is desirable due to the challenge of computing a max operation in the encrypted domain, whereas average is significantly easier to compute.

\begin{table}[]
    \centering
    \begin{tabular}{c c c c c c c}
    \toprule
         & \multicolumn{3}{|c|}{Serial} & \multicolumn{3}{|c|}{Total}\\
        Operation & Adds & Mults & Rots & Adds & Mults & Rots\\
        
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:complexity}
\end{table}


\subsection{Further Attacks}
We reason in Section \ref{sec:intro}\lnote{?} that tolerating byzantine adversaries is not sensical for this problem and that the collusion threat model is reasonable. However, there is an attack outside of the collusion model that we argue is likely to be performed. Instead of sending the resultant ciphertexts at the end of the computation, a mercenary process working with the client could break the privacy of the server by sending ciphertexts containing secret function parameters used to compute $f$. The server would apply its portion of the secret key to the ciphertexts before sending them to the client. The client would then learn private information from the server upon decryption of the ciphertexts. In this \lnote{section}, we discuss three mitigations to these attacks.

\subsubsection{Secret Sharing}
Secret sharing is a well-researched method of providing privacy-preserving computation among a group \cite{}. By splitting the server's secret values into several additive secret shares before encryption, the attack is rendered ineffective. 

\subsubsection{Server Participation}
In our described protocol, the server does not perform any of the computation of the neural network. The server computing the final layer (or several layers) of the neural network locally prevents parameter ciphertexts from being sent to the client.

\subsubsection{Result Checking}
There are circumstances when \fnoutput does not need to be private to the server. This is often the case in classification problems. In settings where this is the case, the server may check the output before returning it to the client. In this case, the server sends $enc(result)$ to the client, which applies its secret key share to the ciphertext. The client sends this to the server, which decrypts it. If the result is of the proper form, it is sent to the client. \lnote{what about dishonest server working with merc? add in random values??}
